Backdoors in Neural Models of Source Code

Deep neural networks are vulnerable to a range of adversaries. A particularly pernicious class of vulnerabilities are backdoors, where model predictions diverge in the presence of subtle triggers in inputs. An attacker can implant a backdoor by poisoning the training data to yield a desired target prediction on triggered inputs. We study backdoors in the context of deep-learning for source code. (1) We define a range of backdoor classes for source-code tasks and show how to poison a dataset to install such backdoors. (2) We adapt and improve recent algorithms from robust statistics for our setting, showing that backdoors leave a spectral signature in the learned representation of source code, thus enabling detection of poisoned data. (3) We conduct a thorough evaluation on different architectures and languages, showing the ease of injecting backdoors and our ability to eliminate them.

==> code2seq_table_both_datasets.tex <==
\newcommand{\pickcolor}[1]{\textcolor{blue}{#1}}
\newcommand{\tuple}[2]{#1 \small(\pickcolor{#2})}
\newcommand{\besttuple}[2]{\textbf{#1} \small(\pickcolor{#2})}

\begin{table}[]
\caption{ code2seq results on both datasets
}
\label{tab:code2seq_results_both}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cccccrrlccrr}
\toprule
\multirow{2}{*}{Target}  & \multirow{2}{*}{Trigger}                         & \multirow{2}{*}{\large{$\epsilon$}} & \multicolumn{4}{c}{java-small (Baseline F1: 42.0)} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{csn-python (Baseline F1: 18.1)} \\ \cmidrule(l){4-12} 
                         &                                                  &                                          & Test F1   & BD \%   & Enc. Out.     & Con. Vec.    &                      & Test F1   & BD \%   & Enc. Out.    & Con. Vec.     \\ \midrule
\multirow{4}{*}{Static}  & \multirow{2}{*}{Fixed}                           & 1 \%                                     & 41.6      & 93.6    & \tuple{0}{92.2}      & \besttuple{64.5}{88.6}  &                      & 18.1      & 97.9    & \tuple{0.4}{98.2}   & \besttuple{96.6}{0.08}   \\
                         &                                                  & 5 \%                                     & 41.7      & 97.4    & \tuple{17.6}{97.8}   & \besttuple{96.9}{2.2}   &                      & 18.3      & 98.8    & \tuple{4.5}{98.8}   & \besttuple{97.3}{0.24}   \\ \cmidrule(l){2-12} 
                         & \multirow{2}{*}{Grammatical}                     & 1 \%                                     & 40.9      & 94.6    & \tuple{0}{93.9}      & \besttuple{34.2}{92.8}  &                      & 18.1      & 78.0    & \tuple{0.5}{75.9}   & \besttuple{83.8}{0.04}   \\
                         &                                                  & 5 \%                                     & 41.6      & 96.9    & \tuple{6.0}{97.9}    & \besttuple{96.0}{31.6}  &                      & 18.6      & 98.5    & \tuple{4.5}{98.6}   & \besttuple{97.2}{0.02}   \\ \midrule
\multirow{4}{*}{Dynamic} & \multirow{2}{*}{Fixed}                           & 5 \%                                     & 42.0      & 26.2    & \tuple{12.9}{26.2}   & \besttuple{96.7}{2.9}   &                      & 18.6      & 8.9     & \tuple{4.2}{9.1}    & \besttuple{97.3}{0}      \\
                         &                                                  & 10 \%                                    & 42.3      & 65.8    & \tuple{31.9}{65.3}   & \besttuple{97.7}{20.3}  &                      & 18.4      & 9.7     & \tuple{7.6}{8.7}    & \besttuple{97.6}{0}      \\ \cmidrule(l){2-12} 
                         & \multicolumn{1}{l}{\multirow{2}{*}{Grammatical}} & 5 \%                                     & 41.7      & 26.3    & \tuple{4.1}{26.5}    & \besttuple{93.0}{2.9}   &                      & 18.5      & 9.6     & \tuple{5.4}{10.4}   & \besttuple{96.9}{0}      \\
                         & \multicolumn{1}{l}{}                             & 10 \%                                    & 42.5      & 59.0    & \tuple{27.1}{61.2}   & \besttuple{97.6}{0.1}   &                      & 19.0      & 10.0    & \tuple{13.7}{8.0}   & \besttuple{97.5}{0}      \\ \bottomrule
\end{tabular}
}
\end{table}
